Fake It Till You Make It: Towards Accurate Near-Distribution Novelty Detection

We aim for image-based novelty detection. Despite considerable progress, existing models either fail or face a dramatic drop under the so-called "near-distribution" setting, where the differences between normal and anomalous samples are subtle. We first demonstrate existing methods experience up to 20% decrease in performance in the near-distribution setting. Next, we propose to exploit a score-based generative model to produce synthetic near-distribution anomalous data. Our model is then fine-tuned to distinguish such data from the normal samples. We provide a quantitative as well as qualitative evaluation of this strategy, and compare the results with a variety of GAN-based models. Effectiveness of our method for both the near-distribution and standard novelty detection is assessed through extensive experiments on datasets in diverse applications such as medical images, object classification, and quality control. This reveals that our method considerably improves over existing models, and consistently decreases the gap between the near-distribution and standard novelty detection performance. The code repository is available at https://github.com/rohban-lab/FITYMI.

==> Figs/Airplane_Fig.tex <==
\begin{figure}[!ht]
    \begin{center}
        \includegraphics[width=13.5cm,height=16cm]{Images/last_air_.jpg}
    \end{center}
    \caption{Generated anomalous samples by different generative models. As opposed to other generative methods, the proposed premature training of the SDE yields authentic, near-distribution, diverse, and artifact-free images. This makes it a better choice for the NND setup.}
\label{SDE_VDE training S_Gpremature , diverse, and AauthenticN}
\end{figure}

==> Figs/KNN_Fig.tex <==
\begin{figure}[!ht]
    \begin{center}
        \includegraphics[width=6cm,height=4cm]{Images/k-change.png}
    \end{center}
    \caption{The effect of changing the number of neighbors on our model's results on ND and NND on the CIFAR-10 dataset. The optimal number of neighbors for each setting is different. Therefore, we chose the number 2 for this parameter, which has the best performance on the ND setting.}\label{Fig:KNN_Effect}
\end{figure}

==> Main/Background.tex <==
The problem of {\it Novelty Detection} for one-class classification is defined using the following setup. Consider $\mathcal{X}$ and $\mathcal{Y}$ be the input and output spaces respectively and let $\mathcal{P}$ be a distribution over $\mathcal{X} \times \mathcal{Y}$. Suppose $\mathcal{F}$ to be a neural network trained on the samples drawn from $\mathcal{P}$ to output a feature representation, which is used to predict the novelty score of an input sample. Let $\mathcal{D}_{\text{Normal}}$ to be the marginal distribution of $\mathcal{P}$ for $\mathcal{X}$. ND aims to define a decision function $\mathcal{G}$, demonstrating the following behavior for an arbitrary given test input $x \in \mathcal{X}$ : 
  \begin{equation}
    \mathcal{G}(x, \mathcal{F})=
    \begin{cases}
      0 & \text{if}\ x \sim \mathcal{D}_{\text{Normal},} \\
      1 & \text{otherwise.}
    \end{cases}
  \end{equation}
For ND  
$|\mathcal{Y}|$ is set to $1$, while for out-of-distribution detection and open-set recognition is $>1$.

==> Main/Intro.tex <==
% The intro writing style should follow this guideline:
% 1st par. Description of the problem area, the core challenge, and the focus of this paper.
% 2nd par. Describe what other methods are done there in this space and particularly wrt the challenge.
% 3rd par. Explain why the problem is not solved yet/still relevant what we propose instead and. Is the challenge deeper or broader, or assumptions too strong? 
% 4th par. Summarize contributions.
% That's it.

% \cs{Too many abbreviations are an unnecessary cognitive burden for the reader. Makes the paper unreadable.}

In anomaly detection (AD) or novelty detection (ND), the objective is to identify test-time samples that are unlikely to come from the training distribution
%, with many applications in manufacturing or healthcare 
\cite{salehi2021unified}. Such samples are called anomalous, while the training set is referred to as normal. Consider $\mathcal{X}$ and $\mathcal{Y}$ to be the input and output spaces respectively, and let $\mathcal{P}$ be a distribution over $\mathcal{X} \times \mathcal{Y}$. Furthermore, let $\mathcal{F}$ be a neural network that is trained on the samples drawn from $\mathcal{P}$ to output a feature representation, which is used to predict the novelty score of an input sample. Let $\mathcal{D}_{\text{Normal}}$ to be the marginal distribution of $\mathcal{P}$ on $\mathcal{X}$. Novelty or anomaly detection aims to define a decision function $\mathcal{G}$ that for any given test input $x \in \mathcal{X}$ returns 0 if $x \sim D_{\text{Normal}}$, and 1 otherwise. It is worth noticing that $|\mathcal{Y}| = 1$, i.e. only one class exists, for the AD and ND. However, it is larger than one for the out-of-distribution detection and open-set recognition. 

Recently, PANDA~\cite{reiss2021panda} and CSI~\cite{tack2020csi} have significantly pushed state-of-the-art and achieved more than 90\% performance on the CIFAR-10 dataset~\cite{krizhevsky2009learning} in the ND task, where one class is assumed to be normal and the rest are considered anomalous. However, most of the their proposed benchmarks mainly focus on detecting abnormal inputs that are semantically far from the normal distribution. In this paper, our focus is on near novelty detection (NND) that is a more challenging task and has been explored to a smaller extent. NND has found several important practical applications in diverse areas such as medical imaging, and  face liveness detection.

%making their detection more valuable since it is a time-consuming and cumbersome task, which even needs high expertise human resources. 

% \cs{This paragraph needs a rewrite without abbreviations and with references to published papers. Praise your peers.}
This problem setup has been recently investigated in the out-of-distribution detection domain by the keyword ``near OOD" detection. SOTA models turned out to be susceptible in making false detection on the anomalous samples that slightly deviate from the normal data. In out-of-distribution detection, due to receiving extra supervision of class labels compared to the novelty detection, a classifier can learn the class boundaries for the in-distribution samples. Such boundaries then come in handy in estimation of the class uncertainty of a given input. Such estimation could be done based on the maximum softmax probability. However, there is no straightforward yet effective solution for the ND or AD tasks (i.e., one-class classification). Besides, in most cases, normal data constitutes less conceptual diversity in the novelty detection setting, making the uncertainty estimation challenging, especially for the close abnormal inputs.   

% \cs{This paragraph is unreadable.}
Our first contribution is to comprehensively benchmark some of the most notable novelty detection methods in the ``near'' novelty detection (NND) setting and demonstrate a significant performance drop of such approaches despite their excellent results on the standard novelty detection tasks. Fig. \ref{fig:NND_Results} compares the performance of PANDA~\cite{reiss2021panda} and CSI~\cite{tack2020csi} in the NND and ND, which shows roughly a 20\% performance drop. Furthermore, while MHRot~\cite{hendrycks2019using} performs quite the same as PANDA and CSI in novelty detection, it works significantly worse in near novelty detection, highlighting the need for a comprehensive near novelty detection benchmarking.

% \cs{Can you rewrite this paragraph without acronyms? Note that we have now three names for our problem: anomaly detection, novelty detection and OOD. If you cannot choose, how do you expect your reader will respond?}
% To cope with the issue in the out-of-distribution domain, \cite{fort2021exploring},  \cite{hendrycks2019using}, and \cite{ruff2019deep} employ outlier exposure techniques, i.e., exposing the model to the real \st{OOD} samples during the training, as an effective while not much expensive way of distinguishing near ODD samples. However, as mentioned in  \cite{kong2021opengan}, they overfit to the available set of training outliers, which are often biased and fail to span the \st{OOD} space exhaustively. Besides, outliers that are placed close to the boundaries of a trained model contribute the most to near \st{OOD} detection, making them less accessible with respect to the arbitrary downstream tasks and expensive to be found on the available datasets.


To cope with the issue in the out-of-distribution domain, \cite{fort2021exploring},  \cite{hendrycks2019using}, and \cite{ruff2019deep} employ outlier exposure techniques, i.e., exposing the model to the real outliers, available on the internet, during training. Such outliers are often inexpensive to acquire and may not be directly relevant to the downstream task. However, as mentioned in \cite{kong2021opengan}, such models tend to overfit to the  training outliers, and become biased and fail to generalize on the entire out-of-distribution space. Besides, outliers that are placed close to the boundaries of a trained model potentially contribute the most to near out-of-distribution detection. However, such samples are less accessible with respect to the arbitrary downstream tasks, and often expensive to acquire. Alternatively, some approaches \cite{kong2021opengan, pourreza2021g2d} utilize GANs to generate outliers. Nevertheless, these generative models suffer from (1) instability in the training phase, (2) poor performance on high-resolution images, and (3) low diversity of generated samples \cite{salehi2021arae}. To address the mentioned challenges, we propose to use a ``non-adaptive''  anomaly data generation method.


\input{Figs/NND_Results}
 

%  \cs{This is a lot of space to present the contributions.}
 
%  Here, to take the advantages of OE techniques, and avoid its downsides such as high cost and the risk of biasing, We have alternatively proposed to generate  anomaly data through state-of-the-art generative models as a proxy of outliers and exposing to such data the  anomaly detectors.  Previously researchers have attended to generating the ODD samples using the inlier samples, and by having such samples learn a detector as a binary classifier as in \cite{zaheer2020old} and \cite{pourreza2021g2d}, or have used generated samples to improve the open set recognition tasks(OpenGAN \cite{kong2021opengan}). Nevertheless, these generative models suffer from (1) instability in the training phase, (2) Work for the low-resolution images, and (3) Low diversity in generated samples \cite{salehi2021arae}. To address the mentioned challenges, we have proposed to use a ``non-adaptive''  anomaly data generation method.
 
 Our second contribution is shedding light on the capabilities of the recently proposed SDE generative models \cite{song2020score}, in the ND domain. By providing comprehensive experiments and visualizations, we show that a prematurely trained SDE model can generate {\it diverse} and {\it non-noisy} near outliers, which significantly beat samples that are generated by GANs or obtained from the available datasets. %when used to boost the performance of ND models. 
 Furthermore, we make it a step further, and demonstrate a large performance drop of roughly 15\% for the methods that employ the outlier exposure technique such as \cite{hendrycks2019using} and \cite{ruff2019deep} when faced with our  generated anomalous samples. This validates our assertion that the outlier exposure technique is incapable of detecting close outlier samples. Finally, we fine-tune simple baseline ND methods with the generated samples to distinguish them from the normal data, and  evaluate our method in the both of ND and NND tasks. This spans wide variety of applications and anomaly granularity. We get consistently and significantly better results on a variety of other NND benchmarks. 


% Finally, We propose a novel tframework that, as opposed to \cite{kong2021opengan}, \cite{ruff2019deep}, \cite{zaheer2020old}, and \cite{pourreza2021g2d} is not confined by the input's resolution, behaves utterly stable during the training process, and works across different datasets with a variety of granularity and applications such as MVTecAD, Weather, WBC, and CIFAR-10 while achieves SOTA results on both of the ND and NND benchmarks by a large margin.
The  key contributions of this paper are:
\begin{itemize}
    \item We explore near distribution novelty detection in the one-class setting for the first time.  Inspired by recent works on the multi-class setting, we defined a benchmark for quantifying similarity between normal and abnormal samples in our one-class scenario and evaluate several notable SOTA methods in the new evaluation setup. 
    \item We show that SDE models can be employed in AD/ND domain to produce high-quality and diverse near distribution anomalous samples. These can be further used to either boost the performance of existing ND methods, or evaluate such methods in the NND setting. It is also shown that the most notable SOTA methods that already use outlier exposure are susceptible to false detection of our generated samples. 
    \item We propose a novel method for anomaly/novelty detection. We introduce discriminating generated fakes and authentic images as a fine-tuning strategy for the novelty detection task. We show that a pre-trained model applied on a defined scheme outperforms SOTA models on both conventional anomaly detection and defined near anomaly detection benchmarks by a large margin up to \textbf{6\%} on some datasets.
\end{itemize}

==> Main/Settings.tex <==
\subsection{Datasets} Following previous works, we evaluate the methods on standard datasets CIFAR-10 \cite{krizhevsky2009learning}, CIFAR-100 \cite{krizhevsky2009learning} and extend the results on small and fine-grained datasets FGVC-Aircraft \cite{maji13fine-grained}, Birds \cite{wah2011caltech}, Flowers \cite{nilsback2008automated}, Stanford-Cars \cite{krause20133d}, MVTecAD \cite{bergmann2019mvtec}, WBC \cite{zheng2018fast}, and Weather \cite{gbeminiyi2018multi}.  For the full dataset descriptions and details see the Appendix\ref{setting}. Following the standard ND protocol, multi-class datasets are converted into an anomaly detection task by setting a class as normal and all other
classes as anomalies. This is performed for all classes, in practice turning a single dataset with C classes into C datasets  \cite{Salehi_2021_CVPR, reiss2021mean, reiss2021panda}. We note that some of the mentioned datasets, such as WBC, FGVC-Aircraft, Stanford-Cars, and Weather,  naturally correspond to the near-ND setup. Also, in an alternative near-ND setup, each class of CIFAR-10 ($C^{10}_{i}$) and its closest class
 %, which will be defined later, 
in CIFAR-100 ($C^{100}_{i}$) are selected. Then, the model is trained on the training samples of ($C^{10}_{i}$) and tested against the aggregation of ($C^{100}_{i}$) and ($C^{10}_{i}$) test sets. Finally, the average AUROC results across datasets is reported.

%\input{Figs/Fid_Score}

==> Main/Social_Impacts.tex <==
The goal of this study is to increase the safety of modern machine learning models. This will benefit a wide range of fields and activities in society. We believe that novelty detection is used in a variety of areas, including financial services (for example, fraud detection), manufacturing (for example, failure detection), and health care (e.g., unseen disease identification). We intend to offer machine learning researchers an easy-to-use tool that provides safety against a wide range of anomalous data in the real world applications through our study and the release of our code. While we do not expect our effort to have any negative implications, we hope to continue to build on our method in future work.

==> Tables/GAN_Fake_Detection.tex <==
\begin{table}[!htb]
  \centering
   \caption{The performance of SOTA methods on the samples generated by StyleGAN2. The results reveal that regardless of employing an SSL loss with heavy augmentations or pre-trained features, fine-tuning the model with near outliers better forms the normal boundaries.}\label{Table:Synthetic_Anomaly_Detection}
 \resizebox{0.7\textwidth}{!}{ 
  \begin{tabular}{lc*{7}{c}} 
  \toprule 
   \multicolumn{1}{c}{Dataset }& \multicolumn{5}{c}{Methods}  \\
   \cmidrule(lr){1-1} \cmidrule(lr){2-7} 
   &{\color{red} ADIB}&CSI &PANDA  &MSAD&Transformaly&Ours  \\  
  \cmidrule(lr){1-1}  \cmidrule(lr){2-7} 
  Cifar-10-FSGAN&55.4 &83.1& 66.1 &69.4&82.2&\textbf{95.1} \\
     \bottomrule
  \end{tabular} }
\end{table} 



\begin{table}[!htb]
  \centering
   \caption{\color{red}OE ablation.}\label{Table:Synthetic_Anomaly_Detection}
 \resizebox{0.7\textwidth}{!}{ 
  \begin{tabular}{lc*{5}{c}} 
  \toprule 
   \multicolumn{1}{c}{Dataset }& \multicolumn{4}{c}{OEs}  \\
   \cmidrule(lr){1-1} \cmidrule(lr){2-5} 
   &{without extra dataset}&+100 data from MNIST &+100 data from SVHN  &+100 data from CIFAR100   \\  
  \cmidrule(lr){1-1}  \cmidrule(lr){2-5} 
  Cifar-10vs100&90.0 &90.2& 90.6 &95.1\\
     \bottomrule
  \end{tabular} }
\end{table} 

==> Tables/ND_Results.tex <==
\begin{table}[!ht]
  \centering
 
  \caption{Performance of anomaly detection methods (AUROC \%) on the far (easy) datasets. In these datasets, images of each class are substantially different from other classes; therefore, the anomaly detection task is more trivial. Our method outperforms the prior methods in these datasets.
  %\newline
      % \centerline{ One class setting}
  }\label{Table:ND_Results}
 \resizebox{\textwidth}{!}{ \begin{tabular}{lc*{5}{c}}
  
    \toprule
   &  Birds &Flowers&  CIFAR-10& CIFAR-100    \\    \toprule
   CSI &52.4& 60.8&   94.3 &89.6  \\
      PANDA  &95.3& 94.1&  96.2 &94.1 \\
      MSAD  &96.7& 96.5& 97.2 &96.4  \\
      Transformaly  &97.8& \textbf{99.9}  & 98.3 &97.3  \\
       \toprule 
       Ours  &\textbf{98.5}& \textbf{99.9} &   \textbf{99.3} &\textbf{98.1}  \\
     \bottomrule
  \end{tabular}}
  
\end{table} 



 

==> Tables/NND_Results.tex <==
\begin{table}[!ht]
  \centering
 
  \caption{Anomaly detection methods performance (AUROC \%) on the near (hard) datasets. In these datasets, images of each class are much more similar to other classes; as a result, the anomaly detection task is more complicated. Our method outperforms the prior methods in most of these datasets.
  %\newline
      % \centerline{ One class setting}
  }\label{Table:NND_Results}
 \resizebox{\textwidth}{!}{ \begin{tabular}{lc*{7}{c}}
  
    \toprule
   & Airplane& WBC& Weather&MvTec & CIFAR-10 vs 100   \\    \toprule
   CSI & 64.6 &  50.4 &91.5& 63.6&76.1    \\
      PANDA & 77.7 &  87.4 &81.5& 86.5&76.8  \\
      MSAD& 79.8 &  87.0 &92.4& 87.2&  79.5  \\
      Transformaly& 84.0  & 85.1 &94.3S&\textbf{87.9}&84.1   \\
       \toprule 
       Ours& \textbf{88.7} & \textbf{91.2} &\textbf{97.0}&86.4 & \textbf{90.3} \\
     \bottomrule
  \end{tabular}}
  
\end{table} 

==> Tables/New_ND_results.tex <==
\hfuzz=0.64pt
\begin{table}[!ht]
  \centering
   \caption{The performance of novelty detection methods (AUROC \%) in the ND setting on various datasets. Our method achieves the SOTA or considerably pass it on almost all the datasets.}\label{Table:s_Stopping}
   \resizebox{\textwidth}{!}{\begin{tabular}{llr*{9}{c}}

 

    \toprule
   \multicolumn{1}{c}{Datasets} & \multicolumn{1}{c}{From Scratch} & \multicolumn{6}{c}{Pre-trained} \\
   \cmidrule(lr){1-1} 
    \cmidrule(lr){2-2}  \cmidrule(lr){3-8}
       & CSI&{  \color{red} PatchCore}&PANDA &MSAD& {\color{red} MSAD}&Transformaly& Ours      \\    
        &{\footnotesize(ResNet-18)}  &{\footnotesize (WideResNet50)} &{\footnotesize(ResNet-152) } & {\footnotesize(ResNet-152)}& {\footnotesize (ViT-B\_16)}&{\footnotesize(ViT-B\_16)} & {\footnotesize (ViT-B\_16) }  \\  
    \cmidrule(lr){1-1} 
    \cmidrule(lr){2-2}  \cmidrule(lr){3-8}
       Birds& 52.4&58.1&95.3&96.7&93.3&97.8&\textbf{98.5}   \\

       CIFAR-10& 94.3&67.2&96.2&97.2&94.1&98.3&\textbf{99.1}   \\ 
        CIFAR-100& 89.6&64.1&94.1&96.4&93.0&97.3&\textbf{98.1}      \\
         Flowers&  60.8&74.8&94.1&96.5 &98.6&\textbf{99.9}&\textbf{99.9}   \\

       MvTecAD&     63.6&\textbf{99.6}&86.5 &87.2&85.5&87.9&86.4    \\ 
     \bottomrule
 
    
    
  \end{tabular}}
\end{table}


==> Tables/Sota_Fake_Results.tex <==
\begin{table}[!htb]
  \centering
 
  \caption{The performance of novelty detection methods (AUROC \%) on our Cifar-10-FSDE dataset that consists of images generated using the proposed method on the CIFAR-10 dataset. Each model is trained according to its corresponding setting, except its test-time anomalies are replaced by our fake samples.
  %\newline  ND
      % \centerline{ One class setting}
  }\label{Table:Sota_Fake_Results}
 \resizebox{\textwidth}{!}{ 
 \begin{threeparttable}{ 
  \begin{tabular}{lc*{8}{c}}
   
  \toprule 
   \multicolumn{1}{c}{Dataset }&\multicolumn{2}{c}{OOD (Multi-Class) } & \multicolumn{7}{c}{ND (One-Class) }  \\
   \cmidrule(lr){1-1}\cmidrule(lr){2-3} \cmidrule(lr){4-10} 
 
   & OpenGAN\tnote{\textdagger}& OE\tnote{\textdagger} &{\color{red} ADIB }\tnote{*}\tnote{\textdagger}&DeepSAD\tnote{\textdagger} &GT&CSI&PANDA\tnote{*}&MSAD\tnote{*}&Transformaly\tnote{*}   \\  
  \cmidrule(lr){1-1} \cmidrule(lr){2-3} \cmidrule(lr){4-10} 
   CIFAR-10-FSDE&  88.4  &78.2& 52.0&53.4   &60.5&87.4&57.7&64.1&75.0  \\
  
 
     \bottomrule
  \end{tabular}}
        \begin{tablenotes}
        \item[*] Pretrained on ImageNet.
        \item[\textdagger] Require extra Dataset.
    \end{tablenotes}
  \end{threeparttable}}
\end{table} 

